Multitechnique testing of the viscous decretion disk model I. The stable and tenuous disk of the late-type Be star $\beta$ CMi

The viscous decretion disk (VDD) model is able to explain most of the currently observable properties of the circumstellar disks of Be stars. However, more stringent tests, focusing on reproducing multitechnique observations of individual targets via physical modeling, are needed to study the predictions of the VDD model under specific circumstances. In the case of nearby, bright Be star $\beta$ CMi, these circumstances are a very stable low-density disk and a late-type (B8Ve) central star. The aim is to test the VDD model thoroughly, exploiting the full diagnostic potential of individual types of observations, in particular, to constrain the poorly known structure of the outer disk if possible, and to test truncation effects caused by a possible binary companion using radio observations. We use the Monte Carlo radiative transfer code HDUST to produce model observables, which we compare with a very large set of multitechnique and multiwavelength observations that include ultraviolet and optical spectra, photometry covering the interval between optical and radio wavelengths, optical polarimetry, and optical and near-IR (spectro)interferometry. Due to the absence of large scale variability, data from different epochs can be combined into a single dataset. A parametric VDD model with radial density exponent of $n$ = 3.5, which is the canonical value for isothermal flaring disks, is found to explain observables typically formed in the inner disk, while observables originating in the more extended parts favor a shallower, $n$ = 3.0, density falloff. Modeling of radio observations allowed for the first determination of the physical extent of a Be disk (35$^{+10}_{-5}$ stellar radii), which might be caused by a binary companion. Finally, polarization data allowed for an indirect measurement of the rotation rate of the star, which was found to be $W \gtrsim 0.98$, i.e., very close to critical.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Own macros
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Astronomical Variables and Observables 
%
\newcommand{\mstar}{\mbox{$M_{\star}$}\xspace}
\newcommand{\rstar}{\mbox{$R_{\star}$}\xspace}
\newcommand{\req}{\mbox{$R_{\rm eq}$}\xspace}
\newcommand{\rpole}{\mbox{$R_{\rm pole}$}\xspace}
\newcommand{\lstar}{\mbox{$L_{\star}$}\xspace}
%
\newcommand{\teff}{\mbox{$T_{\mathrm{eff}}$}\xspace}
\newcommand{\logg}{\mbox{$\log g $}\xspace}
\newcommand{\logeps}{\mbox{$\log\varepsilon$}\xspace} 
\newcommand{\mdot}{\mbox{$\dot{M}$}\xspace}
\newcommand{\vsys}{\mbox{$v_{\mathrm{sys}}$}\xspace}
\newcommand{\vrad}{\mbox{$v_{\mathrm{rad}}$}\xspace}
\newcommand{\vpuls}{\mbox{$v_{\mathrm{puls}}$}\xspace}
\newcommand{\vred}{\mbox{$v_{\mathrm{red}}$}\xspace}
\newcommand{\vviolet}{\mbox{$v_{\mathrm{violet}}$}\xspace}
\newcommand{\vinf}{\mbox{$v_\infty$}\xspace}
\newcommand{\vesc}{\mbox{$v_{\mathrm{esc}}$}\xspace}
\newcommand{\vsini}{\mbox{$v\sin i$}\xspace}
\newcommand{\vrot}{\mbox{$v_{\mathrm{rot}}$}\xspace}
\newcommand{\vcrit}{\mbox{$v_{\mathrm{crit}}$}\xspace}
\newcommand{\vkep}{\mbox{$v_{\mathrm{orb}}$}\xspace}

\newcommand{\omeang}{\mbox{$\omega$}\xspace}
\newcommand{\omelin}{\mbox{$\Upsilon$}\xspace} % as in Cranmer, 2006
\newcommand{\omeorb}{\mbox{$W$}\xspace}

%\newcommand{\wlam}{\mbox{$W_{\lambda}$}\xspace}
\newcommand{\wlam}{\mbox{$\mathit{EW}$}\xspace}
\newcommand{\la}{\mbox{$\lambda$}\xspace}
\newcommand{\bz}{\mbox{$\langle{B_z}\rangle$}\xspace}

\newcommand{\vr}{\mbox{$V\!/R$}\xspace}
\newcommand{\bminv}{\mbox{$B\!-\!V$}\xspace}
\newcommand{\uminb}{\mbox{$U\!-\!B$}\xspace}
\newcommand{\vminr}{\mbox{$V\!-\!R$}\xspace}
%
%        Astronomical units
%
\newcommand{\Mstar}{\mstar}   % Not a unit, but a normalization quantity
\newcommand{\Rstar}{\rstar}   % Not a unit, but a normalization quantity
% Let's do as if the following were SI units  (i.e. in roman):
\newcommand{\Msun}{\mbox{${\mathrm M}_{\odot}$}\xspace}
\newcommand{\Rsun}{\mbox{${\mathrm R}_{\odot}$}\xspace}
\newcommand{\Lsun}{\mbox{${\mathrm L}_{\odot}$}\xspace}
\newcommand{\Myr}{\mbox{${\mathrm M}_{\odot}{\mathrm{yr}}^{-1}$}\xspace}
% SI units:
\newcommand{\micron}{\mbox{$\mu\rm m$}\xspace}
\newcommand{\gcm}{\mbox{$\rm g\,cm^{-3}$}\xspace}
\newcommand{\kms}{\mbox{${\mathrm{km\,s}}^{-1}$}\xspace}
%
\renewcommand{\deg}{\degree\xspace}
%
%       Spectral lines, ions and spectral types
%
\newcommand{\LyB}{\mbox{{{Ly}}$\mathrm{\beta}$}\xspace}
\newcommand{\HA}{\mbox{{H}$\mathrm{\alpha}$}\xspace}
\newcommand{\HB}{\mbox{{H}$\mathrm{\beta}$}\xspace}
\newcommand{\HG}{\mbox{{H}$\mathrm{\gamma}$}\xspace}
\newcommand{\HD}{\mbox{{H}$\mathrm{\delta}$}\xspace}
\newcommand{\HE}{\mbox{{H}$\mathrm{\epsilon}$}\xspace}
\newcommand{\BrG}{\mbox{{Br}$\mathrm{\gamma}$}\xspace}
\newcommand{\Pa}[1]{\mbox{{Pa}$_{#1}$}\xspace}
%
\newcommand{\spec}[3]{\mbox{#1\,{\sc #2}\,$\lambda$#3}\xspace}
\newcommand{\specs}[3]{\mbox{#1\,{\sc #2}\,$\lambda\lambda$#3}\xspace}
\newcommand{\ion}[2]{\mbox{#1\,{\sc #2}}\xspace}
%
\newcommand{\spt}[2]{\mbox{#1\,#2}\xspace}
%
%       Objects
%
\newcommand{\alpara}{\mbox{$\mathrm{\alpha}$}~Ara\xspace}
\newcommand{\alperi}{\mbox{$\mathrm{\alpha}$}~Eri\xspace}
\newcommand{\betcep}{\mbox{$\mathrm{\beta}$}~Cep\xspace}
\newcommand{\betlyr}{\mbox{$\mathrm{\beta}$}~Lyr\xspace}
\newcommand{\gamcas}{\mbox{$\mathrm{\gamma}$}~Cas\xspace}
\newcommand{\delsco}{\mbox{$\mathrm{\delta}$}~Sco\xspace}
\newcommand{\omeori}{\mbox{$\mathrm{\omega}$}~Ori\xspace}
\newcommand{\mucen}{\mbox{$\mathrm{\mu}$}~Cen\xspace}
\newcommand{\etacen}{\mbox{$\mathrm{\eta}$}~Cen\xspace}
\newcommand{\lameri}{\mbox{$\mathrm{\lambda}$}~Eri\xspace}
\newcommand{\omecma}{\mbox{$\mathrm{\omega}$}~CMa\xspace}
\newcommand{\kapcma}{\mbox{$\mathrm{\kappa}$}~CMa\xspace}
\newcommand{\epscap}{\mbox{$\mathrm{\epsilon}$}~Cap\xspace}
\newcommand{\zettau}{\mbox{$\mathrm{\zeta}$}~Tau\xspace}
\newcommand{\phiper}{\mbox{$\mathrm{\varphi}$}~Per\xspace}
\newcommand{\piaqr}{\mbox{$\mathrm{\pi}$}~Aqr\xspace}
\newcommand{\psiper}{\mbox{$\mathrm{\psi}$}~Per\xspace}
\newcommand{\feper}{\mbox{$48$}~Per\xspace}
\newcommand{\felib}{\mbox{$48$}~Lib\xspace}
\newcommand{\betcmi}{\mbox{$\mathrm{\beta}$}~CMi\xspace}
\newcommand{\delcen}{\mbox{$\mathrm{\delta}$}~Cen\xspace}
\newcommand{\etatau}{\mbox{$\mathrm{\eta}$}~Tau\xspace}
\newcommand{\kapdra}{\mbox{$\mathrm{\kappa}$}~Dra\xspace}
\newcommand{\pcar}{\mbox{$\mathrm{p}$}~Car\xspace}
\newcommand{\alpcol}{\mbox{$\mathrm{\alpha}$}~Col\xspace}
\newcommand{\xioph}{\mbox{$\mathrm{\chi}$}~Oph\xspace}
\newcommand{\upscyg}{\mbox{$\mathrm{\upsilon}$}~Cyg\xspace}
\newcommand{\betpsc}{\mbox{$\mathrm{\beta}$}~Psc\xspace}
\newcommand{\omicas}{\mbox{$\mathrm{\omicron}$}~Cas\xspace}
\newcommand{\sixcep}{\mbox{$\mathrm{6}$}~Cep\xspace}
\newcommand{\omiaqr}{\mbox{$\mathrm{\omicron}$}~Aqr\xspace}
\newcommand{\thecrb}{\mbox{$\mathrm{\vartheta}$}~CrB\xspace}
\newcommand{\onedel}{\mbox{$1$}~Del\xspace}
\newcommand{\betmon}{\mbox{$\beta^1$}~Mon\xspace}
\newcommand{\omecar}{\mbox{$\omega$}~Car\xspace}
%
% Codes, Models, Instruments
%
\newcommand{\bruce}{{\sc bruce/kylie}\xspace}
\newcommand{\hdust}{{\sc hdust}\xspace}
\newcommand{\fastrot}{{\sc fas\-trot}\xspace}
\newcommand{\charron}{{\sc charron}\xspace}
\newcommand{\bedisk}{{\sc bedisk}\xspace}
\newcommand{\simeca}{{\sc simeca}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Fancy stuff 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\lgrey{\color{black!30!white}}
%\def\grey{\color{black!60!white}}
%\def\green{\color{green}}
%\def\textgreen{\color{ForestGreen}}
%\def\black{\color{black}}
%\def\red{\color{red}}
%\def\blue{\color{blue}}
%\def\yellow{\color{yellow}}
%\def\white{\color{white}}
%\def\magenta{\color{magenta}}
%\definecolor{beige}{HTML}{FFDF8C}
%\def\beige{\color{beige}}
%\def\gold{\color{Olive}}
%
%\newcommand{\draft}[1]{{{\bf\sf\red Draft:}\grey\sf\ #1}\xspace}
%\newcommand{\TRi}[1]{{{\bf\sf\red Rivi:}\grey\sf\ #1}\xspace}
%\newcommand{\TRi}[1]{{{}}}


